Joint Antenna Position and Beamforming Optimization with Self-Interference Mitigation in MA-ISAC System

Movable antennas (MAs) have demonstrated significant potential in enhancing the performance of integrated sensing and communication (ISAC) systems. However, the application in the integrated and cost-effective full-duplex (FD) monostatic systems remains underexplored. To address this research gap, we develop an MA-ISAC model within a monostatic framework, where the self-interference channel is modeled in the near field and characterized by antenna position vectors. This model allows us to investigate the use of MAs with the goal of maximizing the weighted sum of communication capacity and sensing mutual information. The resulting optimization problem is non-convex making it challenging to solve optimally. To overcome this, we employ fractional programming (FP) to propose an alternating optimization (AO) algorithm that jointly optimizes the beamforming and antenna positions for both transceivers. Specifically, closed-form solutions for the transmit and receive beamforming matrices are derived using the Karush-Kuhn-Tucker (KKT) conditions, and a novel coarse-to-fine grained search (CFGS) approach is employed to determine the high-quality sub-optimal antenna positions. Numerical results demonstrate that with strong self-interference cancellation (SIC) capabilities, MAs significantly enhance the overall performance and reliability of the ISAC system when utilizing our proposed algorithm, compared to conventional fixed-position antenna designs.

==> formula-part.tex <==
% \section{System model}

% \subsection{$H_{SI}$ model}

% \textbf{Near field LOS model:}
% \begin{equation}
% \mathbf{H}(n_1, n_2) = \frac{1}{r_{n_1, n_2}} e^{-j \frac{2\pi}{\lambda} r_{n_1, n_2}},
% \end{equation}


% \begin{equation}
% \begin{split}
% r(x_i,y_j) = & \sqrt{r^2 + x_i^2 + y_j^2 + 2ry_j\sin(\theta-\phi) \\
% & - 2rx_i\sin\theta - 2x_iy_j\cos\phi}
% \end{split}
-% \end{equation}




% \begin{equation}
% \mathbf{R(x,y)} = \begin{bmatrix}
% r(x_1,y_1) & \cdots  & r(x_1,y_{N_R}) \\
% \vdots & \ddots  &\vdots \\
% r(x_{N_T},1) & \cdots  & r(x_{N_T},y_{N_R})
% \end{bmatrix}
% \end{equation}

% \begin{equation}
% \begin{split}
% H_{SI} = & \mathbf{H}_{LOS}(R(\mathbf{x},\mathbf{y}),\theta,\phi) \\
% = & \begin{bmatrix}
% H(x_1,y_1) & \cdots  & H(x_1,N_R) \\
% \vdots & \ddots  & \vdots \\
% H(x_{N_T},y_1) & \cdots  & H(x_{N_T},y_{N_R})
% \end{bmatrix}\in \mathbb{C}^{N_T \times N_R}
% \end{split}
% \end{equation}


% After channel estimation to obtain $\theta,\phi$, $H_{SI}=V(\mathbf{x,y})$.

% \subsection{Communication part model}
% \begin{equation}
% \mathbf{h}_k(\mathbf{x}) = \sqrt{\frac{N_t}{L_p}} \sum\limits_{l=1}^{L_p} \rho_{k,l} \mathbf{a}_{k,l}(\mathbf{x})\in \mathbb{C}^{N_T \times 1}
% \end{equation}

% Steering vector:
% \begin{equation}
% \small
% \mathbf{a}_{k,l}(\mathbf{x}) = \begin{bmatrix} 1 & e^{j\frac{2\pi }{\lambda} x_1\cos(\theta)}  & \cdots & e^{j\frac{2\pi }{\lambda} x_{N_T}\cos(\theta)} \end{bmatrix}^T\in \mathbb{C}^{N_T \times 1}
% \label{steering_vector}
% \end{equation}

% Precoding matrix:
% \begin{equation}
% \mathbf{F}=[\mathbf{f_1},\mathbf{f_2},...,\mathbf{f_K}]\in \mathbb{C}^{N_T \times K}
% \end{equation}
% The power for each antenna can be defined as:

% \begin{equation}
% \mathbf{\bar{f}}(n)=[f_1(n),...,f_K(n)]^T\in \mathbb{C}^{K \times 1}
% \end{equation}

% \begin{equation}
% \hat{\mathbf{f}}=[\|\mathbf{\bar{f}}(1)\|_2, ...,\|\mathbf{\bar{f}}(N_T)\|_2]^T\in \mathbb{C}^{N_T \times 1}
% \end{equation}

% For K users, signals are $\mathbf{s}=[s_1,s_2,...,s_K]^T\in \mathbb{C}^{K \times 1}$, used both for sensing and communication:
% \begin{equation}
% y_k = \mathbf{h}_k^H(x)\mathbf{f_k}s_k + \mathbf{h}_k^H\sum\limits_{j=1, j\neq k}^{K} \mathbf{f}_j s_j + n_k \in\mathbb{C}
% \end{equation}

% \begin{equation}
% R_k=\log_2(1+\text{SINR}_k)
% \end{equation}

% \begin{equation}
% \text{SINR}_k = \frac{|\mathbf{h}_k^H(x)\mathbf{f}_k|^2}{\sum\limits_{j=1, j \neq k}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + \sigma_k^2}
% \end{equation}

% \subsection{Sensing part model (with no clutters)}
% Current transmitted signals are still $\mathbf{s}$.
% Received signal before received beamforming:
% \begin{equation}
% \mathbf{y_{0s}} = \alpha_s \mathbf{b}_s(\mathbf{y}) \mathbf{a}_s^H(\mathbf{x}) \mathbf{F} \mathbf{s}  + \mathbf{H_{SI}} 
%    (\mathbf{x},\mathbf{y})\mathbf{F} \mathbf{s}+\mathbf{n_s}\in \mathbb{C}^{N_R \times 1}
% \end{equation}

% Received signal after received beamforming:
% \begin{align}
% y_{1s} &= \mathbf{w_r}^H  \mathbf{y_{0s}} \notag \\
% &= \alpha_s \mathbf{w_r}^H \mathbf{b}_s(\mathbf{y}) \mathbf{a}_s^H(\mathbf{x}) \mathbf{F} \mathbf{s} \notag \\
% &\quad + \mathbf{w_r}^H \mathbf{H_{SI}}(\mathbf{x}, \mathbf{y}) \mathbf{F} \mathbf{s} \notag \\
% &\quad + \mathbf{w_r}^H \mathbf{n_s} 
% \end{align}

% \begin{equation}
% \text{SINR}_s = \frac{|\alpha_s\mathbf{w_r}^H \mathbf{b}_s(\mathbf{y})\mathbf{a}_s^H(\mathbf{x}) \mathbf{F}|^2}{|\mathbf{w_r}^H H_{SI}(\mathbf{x},\mathbf{y})\mathbf{F}|^2+ \sigma_s^2}
% \end{equation}

% \begin{equation}
% R_s = \log_2(1 + \text{SINR}_s)
% \end{equation}

% $\left\|\mathbf{w_r}\right\|^2=1,\mathbf{a}_s(\mathbf{x})\in \mathbb{C}^{N_T \times 1},\mathbf{b}_s(\mathbf{y})\in \mathbb{C}^{N_R \times 1} $ are steering vectors for transmitter and receiver respectively. (Their forms are similar to Formula.\ref{steering_vector})
% \clearpage
% \newpage

% \section{Optimization problem}
% \begin{equation}
% \text{(P1)} \quad \max_{\mathbf{F}, \mathbf{x},\mathbf{y},\mathbf{w_r}} \mathcal{G}(\mathbf{F}, \mathbf{x},\mathbf{y},\mathbf{w_r}) = \varpi_c \sum\limits_{k=1}^{K} R_k + \varpi_s R_s,
% \label{optimizationproblem}
% \end{equation}

% \begin{equation}
% \text{s.t.} \quad \text{Tr}(\mathbf{F}^H \mathbf{F}) \leq P_0, E{\{ss^H\}}=\mathbf{I},\left\|\mathbf{w_r}\right\|^2=1
% \end{equation}

% \begin{equation}
% P_{PA} + P_A \|\hat{\mathbf{f}}\|_0 \leq P_{tot}
% \end{equation}

% \begin{equation}
% \mathbf{x} \in \mathcal{A}, \mathbf{y} \in \mathcal{B}, |x_a-x_b|\geq D_0,|y_c-y_d|\geq D_0
% \end{equation}


% The problem(\ref{optimizationproblem}) is equivalent to P2 with Lagrangian dual transform (to be proofed)

% \begin{align}
%     \text{(P2)} &\quad \mathcal{G}_d(\mathbf{F}, \mathbf{x},\mathbf{y},\mathbf{w_r},\mu) =  \varpi_c \sum\limits_{k=1}^{K} log_2(1+\mu_k) + \varpi_s log_2(1+\mu_{K+1}) - \varpi_c \sum\limits_{k=1}^{K} \mu_k - \varpi_s \mu_{K+1} \notag \\ 
%     & + \varpi_c\sum\limits_{k=1}^{K}\left(\frac{(1+\mu_k)|\mathbf{h}_k^H(x)\mathbf{f}_k|^2}{\sum\limits_{j=1}^{K} |\mathbf{h}_k^H(x)\mathbf{f}_j|^2 + \sigma_k^2} \right) \\
%     &+\varpi_s \frac{|\alpha_s\mathbf{w_r}^H \mathbf{b}_s(\mathbf{y})\mathbf{a}_s^H(\mathbf{x}) \mathbf{F}|^2}{\sum_{c=1}^C|\alpha_c\mathbf{w_r}^H \mathbf{b}_c(\mathbf{y})\mathbf{a}_c^H(\mathbf{x}) \mathbf{F}|^2 
%     +|\alpha_s\mathbf{w_r}^H \mathbf{b}_s(\mathbf{y})\mathbf{a}_s^H(\mathbf{x}) \mathbf{F}|^2 
%     + |\mathbf{w_r}^H H_{SI}(\mathbf{x},\mathbf{y})\mathbf{F}|^2+ ||w_r||^2\mathbf{\sigma_s}^2}  \notag\\
%     & = \varpi_c \sum\limits_{k=1}^{K} log_2(1+\mu_k) + \varpi_s log_2(1+\mu_{K+1}) - \varpi_c \sum\limits_{k=1}^{K} \mu_k - \varpi_s \mu_{K+1} \notag  \\
%     & +\varpi_c\sum_{k=1}^{K}\left(2\sqrt{1+\mu_k}Re\{\xi^c_k h_k^H(x)f_k(x)\}-|\xi^c_k|^2\left(\sum_{j=1}^K|h_k^H(x)f_j|^2+\sigma_k^2\right)\right) \notag \\
%     & + \varpi_s [ 2\sqrt{1+\mu_{K+1}}Re\{\alpha_s w_r^H b_s(y)a_s^H(x)F\xi^s\} \notag \\
%     &-||\mathbf{\xi}^s||^2\left(\sum_{c=1}^C||\alpha_c w_r^H b_c(y) a_c^H(x)F||^2+||w_r^H H_{SI}^H(x,y)F||^2+||\alpha_s w_r^H b_s(y)a_s^H(x)F||^2+||w_r||^2 \mathbf{\sigma}_s^2\right)]
% \end{align}

% in which,
% \begin{align*}
%     \Lambda_k &= \varpi_c HH^H  + \varpi_s ||\xi^s||^2 \Bigg[
%     \sum_{c=1}^C |\alpha_c|^2 \left(w_r^H b_c(y) a_c^H(x) \right)^H \left(w_r^H b_c(y) a_c^H(x) \right) \\
%     &\quad + |\alpha_s|^2 \left(w_r^H b_s(y) a_s^H(x) \right)^H \left(w_r^H b_s(y) a_s^H(x) \right)  + \left(w_r^H H_{SI}^H(x,y)\right)^H \left(w_r^H H_{SI}^H(x,y)\right) 
%     \Bigg]
% \end{align*}

% \begin{equation*}
% \phi_k=\varpi_c\sqrt{1+\mu_k}\xi^{c(t)*}h_k(x^{(t)})+\varpi_s\sqrt{1+\mu_{K+1}} \alpha_s^{*}\xi^{s(t)*}_k a_s(x^{(t)})b^H_s(y) w_r
% \end{equation*}

% \begin{equation}
%     B=\varpi_c\sum^K_{k=1}ln(1+\mu_k)+\varpi_s ln(1+\mu_{K+1})-\varpi_c\sum_{k+1}\mu_k-\varpi_s\mu_{K+1}-\varpi_c\sum^K|\xi^c_k|^2\sigma_k^2-\varpi_s||\xi^2||...
% \end{equation}
% and with quadratic transform, the sum-of-ratio term can be transformed into ,and 
% \clearpage
% \newpage

% \begin{align}
% \nabla L_{w_r} = \varpi_s & \left\{ \sqrt{\mu_{K+1}+1} \alpha_s^* b^*_s(y) a_s(x) F^* \xi^{s*} \right. \nonumber \\
% & - ||\xi^s||^2 \left( \sum_{c=1}^C |\alpha_c|^2 \left( b_c(y) a_c^H(x) F \right)^* \left( b_c(y) a_c^H(x) F \right)^T w_r^* \right. \nonumber \\
% & + (H_{SI}^H(x,y) F)^* (H_{SI}^H(x,y) F)^T w_r^* \nonumber \\
% & + |\alpha_s|^2 (b_s(y) a_s^H(x) F)^* (b_s(y) a_s^H(x) F)^T w_r^* \nonumber \\
% & \left. \left. + w_r^* \mathbf{\sigma}_s^2 \right) \right\}
% \end{align}

% \begin{align}
%     \Psi&=||\xi^s||^2\left\{\sum|\alpha_c|^2\left(b_c(y)a_c^H(x)F\right)\left(b_c(y)a_c^H(x)F\right)^H+\left(H_{SI}^H(x,y)F\right)\left(H_{SI}^H(x,y)F\right)^H \right. \nonumber\\
%     & \left. +|\alpha_s|^2\left(b_s(y)a_s^H(x)F\right)\left(b_s(y)a_s^H(x)F\right)^H+\sigma_x^2I\right\}
% \end{align}

% \begin{equation}
%        \Delta=\sqrt{1+\mu_{K+1}}\alpha_sb_s(y)a_s^H(x)F\xi^s
% \end{equation}

% \begin{equation}
%     w_r=\left\{\left\{\Psi\right\}^{-1}\right\}^*
%     \left\{\Delta\right\}\nonumber \\
% \end{equation}


% \begin{align}
%     &w_r=\left\{\left\{||\xi^s||^2\left(\sum|\alpha_c|^2\left(b_c(y)a_c^H(x)F\right)\left(b_c(y)a_c^H(x)F\right)^H+\left(H_{SI}^H(x,y)F\right)\left(H_{SI}^H(x,y)F\right)^H\nonumber \right.\right.\right.\\
%     & \left.\left.\left.+|\alpha_s|^2\left(b_s(y)a_s^H(x)F\right)\left(b_s(y)a_s^H(x)F\right)^H+\sigma_x^2I\right)\right\}^{-1}\right\}^*
%     \left\{\sqrt{1+\mu_{K+1}}\alpha_sb_s(y)a_s^H(x)F\xi^s\right\}\nonumber \\
% \end{align}

% \begin{align}
%     &\mathbf{\xi}^{s(t+1)}=\frac{\sqrt{1+\mu_{K+1}}\alpha_s^* w_r^Tb_s^*(y)a_s^T(x)F^*}{I_M+||w_r||^2 \mathbf{\sigma}_s^2} \nonumber\\
% \end{align}

% \begin{equation}
%     I_M=\sum_{c=1}^C||\alpha_c w_r^H b_c(y) a_c^H(x)F||^2+||w_r^H H_{SI}^H(x,y)F||^2+||\alpha_s w_r^H b_s(y)a_s^H(x)F||^2
% \end{equation}

% \begin{equation}
%     I_M=\sum_{c=1}^C||\alpha_c w_r^H b_c(y) a_c^H(x)F||^2+||w_r^H H_{SI}^H(x,y)F||^2+||\alpha_s w_r^H b_s(y)a_s^H(x)F||^2
% \end{equation}

% % \begin{equation}
% %     \beta=\left[ \frac{\sqrt{G_l}\lambda}{4 \pi d_{u,k}} \right]^2
% % \end{equation}

% \begin{equation}
%     c^2_{kj}=\beta_0d_{kj}^{-\alpha_0}
% \end{equation}
% \begin{equation}
%     \alpha \sim \mathcal{CN}\left(0, \frac{c^2_{kj}}{L_p}\right)
% \end{equation}




% \clearpage
% \newpage

% \begin{table}[h]
% \centering
% \caption{Parameters of the FD ISAC system} % 表格标题
% \label{table:1}
% \begin{tabular}{ccc}
% \toprule
% Parameter & Notation & Value \\
% \midrule
% user clutter angle& &$[0,\pi]$\\
% Carrier frequency &$f_c$& 2.4 GHz\\
% Wavelength & $\lambda$ & 0.125 m\\
% Distance between user and BS & $d_{u,b}$ &  [50m,80m]\\
% Distance between object and BS & $d_{u,b}$ &  [10m,20m]\\
% Distance between RX and TX & $d_{TX,RX}$ & 1.25 m\\
%   &$\beta_0$& -40\\
% Pathloss exponent  &$\alpha_0$&2.8\\
% Transmit power  &$P_t$&15 dBm\\
% Receive noise power  &$\sigma_r^2$&-80 dBm\\

% \bottomrule
% \end{tabular}
% \end{table}


% \section{Remaining Problems}
% Unsolved:
% \begin{enumerate}[label=\arabic*)]
%     \item needs one graph for the system model and one graph for the near-field model
%     \item need one paper use only use the beamforming method instead of physical isolation in propagation domain
%     \item D1 how to define?
%     \item Shall we add SI channel K (match to the real scenario)?
% \end{enumerate}
% Solved:
% \begin{enumerate}[label=\arabic*)]
%     \item any constraints for receiving beamforming matrix
%     \item has not added the antenna selection condition
%     \item do not add the receive beamforming matrix(be careful about the dimension)
% \end{enumerate}

==> paper-part.tex <==
\section{Introduction}
\noindent\textbf{Outline:} (about one page)
\begin{itemize}
    \item the importance of isac and MA in 6G
    \item inband full-duplex communication system is a typical scenario in isac which should be considered
    \item self-interfere can be suppressed by MA
    \item our contributions
\end{itemize}
\textbf{Paragraph 1: ISAC in 6G}
\begin{enumerate}
    \item the importance of ISAC in 6G
\end{enumerate}

\textbf{Paragraph 2: MA in ISAC}
\begin{enumerate}
    \item beamforming design is of importance in ISAC
    \item To make full use of the DOF, MA is adopted to overcome the constraints of FPA and AS.
    \item MA use flexible RF chain...(brief intro of principle)
    \item MA can enhcance the capacity by optimization
\end{enumerate}

\textbf{Paragraph 3: Related works}
\begin{enumerate}
    \item MA has shown effectiveness in improving the QOS,..., ISAC 
    \item how previous studies combine ISAC and MA, eg.[UESTC,...]. 
    \item They do not consider a monostatic scenario, this paper pioneered the investigation in dual-functional radar and communication(DFRC), which is typical in ISAC problem
    \item self-interference(SI) is a key problem and how to suppress it using MA
    \begin{itemize}
        \item the importance of supressing SI 
        \item Different from physical isolation, Tx and RX beamforming can suppress the interference actively.[In-Band Full-Duplex Survey] 
        \item MA can be used to further suppress the interference.
        \item We model the SI channel as near-field[UESTC:star..., RIS] and derive the formulas with transmit and receive antennas positions.
    \end{itemize}
\end{enumerate}

\textbf{Paragraph 4: Contributions}

Our contributions can be three folded:
\begin{itemize}
    \item we model the SI channel using  transmitter-receiver's antenna position vector and use MA to further suppress the SI
    \item we propose xxx to jointly optimize the transmit, receive beamforming matrix and the TX/RX antenna positions under DFRC-ISAC scenario.
    \item Numerical results show the effectiveness of our algorithm.
\end{itemize}



\section{System model}
\noindent\textbf{Outline:} (about a half page) The section introduces: Inband full-duplex communication system 

\begin{itemize}
\item  Channel model and signal model
\item  Self-interference channel model under movable antenna system
\item  Metrics for communication and sensing and the final object function
\end{itemize}

\textbf{Paragraph 1: Introduce the relative location of the BS }
\begin{enumerate}
\item  Consider a mono-static in-band full-duplex communication system.
\begin{figure}[h] % 'h' 表示将图片尽量放置在当前位置（here）
    \centering % 使图片居中
    \includegraphics[width=0.25\textwidth]{figs/system model-old.png} % 调整图片宽度
    \caption{system model} % 图片标题
    \label{fig:system modelold} % 图片标签，用于引用
\end{figure}
\end{enumerate}
\subsection{Channel model}
\textbf{Paragraph 1: Introduce channel between BS and User}
\begin{enumerate}

\item The positions of transmit MAs and receive MAs are demoted as $X=[x_1,...,x_{N_T}]^T$ and $Y=[y_1,...,y_{N_R}]^T$.
\item According to the far-response model[zhang], the channel vector for each user can be expressed as xxx


\end{enumerate}
\textbf{Paragraph 2: Introduce near-field channel model using MA}
\begin{enumerate}
    \item introduce  a figure specifically shows the structure of the transceivers' relative positions 
    \item The formulas under MA problem
    \hl{near-field how to consider the space loss??? only a d is not enough}
\end{enumerate}

\subsection{Signal model}

\textbf{Paragraph 1: Introduce signal and communication model and SINR}
\begin{enumerate}
\item $s$ denotes the signal for K user, it can be used for both communication and sensing.
\item $W_t$ is the transmitting beamforming matrix, the baseband received signal at user k is xxx
\item the communication metric is SINR 
\end{enumerate}


\textbf{Paragraph 2: Introduce sensing model and SCNR}
\begin{enumerate}
\item $W_r$ is the combining matrix, the received signal is XXX
\item the sensing metric is SCNR
\end{enumerate}

\subsection{Problem formulation}
\textbf{Paragraph 1: Introduce weighted sum of SINR and SCNR }
\begin{enumerate}
\item the movable range of antennas
\item introduce $\varpi_c, \varpi_s$ 
\item the final metric
\end{enumerate}


\section{Algorithm}
\noindent\textbf{Outline:} (about two page) Subproblem formulas

\begin{enumerate}
\item use quadrature form to transform the formula into 
\item use AO method to update the parameters.
\begin{itemize}
\item subproblems
\item use quadratic transform to get the quadrature form
\end{itemize}
\item solutions for subproblems
\begin{itemize}
    \item Updating Transmit Beamforming,receive combination matrix
    \item Updating Auxiliary Variable for Quadratic Transform
    \item Updating x,y
    \item search algorithm (initial point search)
\end{itemize}
\end{enumerate}
\textbf{Paragraph 1: we use AO to optimize these parameters}
\begin{enumerate}
    \item it is challenging to solve the non-convex problem directly. Thus, we use AO to divide the problem into several subproblems
\end{enumerate}
\subsection{transmit and receive beamforming matrix optimization}
\textbf{Paragraph 1: target of this section}
\begin{enumerate}
    \item We optimize the transmit and receive beamforming matrix F and $W_r$ with fixed x,y and auxiliary variables
\end{enumerate}
\textbf{Paragraph 2: how to get F}
\begin{enumerate}
    \item Sub problem 1 optimize F 
    \begin{itemize}
        \item formula
        \item We can use Lagrange dual method to transform the problem and get the dual problem L=....
        \item By using KKT condition, we can get a closed form of F, which is 
        \item $\lambda$ can be found use bisection method
    \end{itemize}
\end{enumerate}

\textbf{Paragraph 3: how to get $W_R$}
\begin{enumerate}
    \item Similarly we use KKT condition to get the closed for of $W_R$
\end{enumerate}

\subsection{Auxiliary Variables Optimization}

\textbf{Paragraph 1: subproblem 2}
\begin{enumerate}
    \item the closed form of the parameters
\end{enumerate}

\textbf{Paragraph 2: Accordingly, beamforming matrix and auxiliary variables can be alternately }

\subsection{Antennas' Positions Optimization}
\textbf{Paragraph 1: target}
\begin{enumerate}
    \item x,y are optimized with fixed beamformer and auxiliary variables
    \item we propose a random-search method to 
\end{enumerate}





\section{Numerical results}
\noindent\textbf{Outline:} (about one and a half page) the experiment details
\textbf{Paragraph 1: a summery sentence: verify the effectiveness}

\textbf{Paragraph 2: introduce the experiment setup}

\textbf{Paragraph 3: introduce different algorithm }
\begin{enumerate}
    \item BF,FPA;SPGA,MA;DGA(direct gradient decent without initial search),MA
\end{enumerate}

\textbf{Paragraph 4: fig power and objective function}
\begin{figure}[h] % 'h' 表示将图片尽量放置在当前位置（here）
    \centering % 使图片居中
    \includegraphics[width=0.45\textwidth]{figs/power-objective.png} % 调整图片宽度
    \caption{power-objective} % 图片标题
    \label{fig:power-objective} % 图片标签，用于引用
\end{figure}

\textbf{Paragraph 5: fig moving range}
\begin{enumerate}
    \item \hl{how to show x and y??? use a 3D figure?or just split into two figures?}
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{figs/moving range.png}
    \caption{moving rang}
    \label{fig:moving_rang}
\end{figure}

\textbf{Paragraph 6: fig different weights}
\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{figs/different_weight.png}
    \caption{different weight}
    \label{fig:different_weight}
\end{figure}





\section{Conclusion}
(about a half page)
